Generalizing Across Domains via Cross-Gradient Training

We present CROSSGRAD, a method to use multi-domain training data to learn a classifier that generalizes to new domains. CROSSGRAD does not need an adaptation phase via labeled or unlabeled data, or domain features in the new domain. Most existing domain adaptation methods attempt to erase domain signals using techniques like domain adversarial training. In contrast, CROSSGRAD is free to use domain signals for predicting labels, if it can prevent overfitting on training domains. We conceptualize the task in a Bayesian setting, in which a sampling step is implemented as data augmentation, based on domain-guided perturbations of input instances. CROSSGRAD parallelly trains a label and a domain classifier on examples perturbed by loss gradients of each other's objectives. This enables us to directly perturb inputs, without separating and re-mixing domain signals while making various distributional assumptions. Empirical evaluation on three different applications where this setting is natural establishes that (1) domain-guided perturbation provides consistently better generalization to unseen domains, compared to generic instance perturbation methods, and that (2) data augmentation is a more stable and accurate method than domain adversarial training.

==> model.tex <==

\section{Sunita's old notes}
%
As reflected in the network, $y$ is not independent of $d$ given $\vx$. 

A sufficient way to build a domain-independent model for $\Pr(y|\vx)$ is by designing a network $F(\vx)$ to extract content features $\vf$ from $\vx$.  Since $\vf$ is independent of the domain, the $\Pr(y|\vf)$ classifier will then trivially generalize to new domains.  Domain adversarial training can be thought of as attempting exactly that.  Unfortunately, this method does not provide any guarantees that $F(\vx)$ would not overfit on the training domains.

One challenge to designing the sampling process is that the $\Pr(\vx|\vg,y)$ distribution is complicated.  We therefore limit ourselves to sampling around small neighborhoods of training instances as follows: Let $(\vx_i,y_i)$ be a training instance from a domain $d_i$.

We design a sampler to generate a new sample $(\vx', y_i)$ by sampling near $\vg_i$ a nearby $\vg'$ following $\Pr(\vg)$ and then sampling a $\vx'$ from $\Pr(\vx | \vg', y_i)$.  



We instead propose to model the posterior by integrating over the domains as follows

\begin{equation}
\Pr(y|\vx)=\sum_{d\in \cD}\Pr(y|\vx,d)\Pr(d|\vx) = \int_\vg \Pr(y|\vx,\vg)\Pr(\vg|\vx)
\end{equation}

% \sid{I guess we won't actually do any integration, but just rely on the network to predict $\vg^* = \argmax_{\vg} \Pr(\vg|\vx)$ and approximate $\Pr(\vg^*|\vx) \approx 1$, i.e. $\Pr(y|\vx) \approx \Pr(y|\vx,\vg^*)$. Should we clarify this, and can it be somehow exploited below?}
% \sunita{Yes, I agree.  We could justify that way.  Just had a discussion with Preethi, and am inclined to separate out the Bayesian approach from Cross-gradient as two separate pieces of work.}

We next discuss various ways of estimating $\Pr(y|\vx,\vg)$ and $\Pr(\vg|\vx)$ using the training data $L$.  In the training data both $d$ and $y$ are observed, so we maximize the likelihood
\begin{equation}
\Pr(y,d|\vx)= \int_\vg \Pr(y|\vx,\vg)\Pr(\vg|\vx)\Pr(d|\vg)
\end{equation}
% \paragraph{Estimating $\Pr(\vg|\vx)$}
We use a task-dependent neural network $G(\vx)$ to extract $\vg$ from $\vx$, and a softmax layer to convert $\vg$ to $d$. The $\Pr(y|\vx,\vg)$ distribution is modeled by the main classification neural network $C(\vx, \vg) \mapsto y$.

With the domain represented as a continuous vector, we can use various techniques to prevent $C$ from over-fitting on the training domains.

\todo{Propose methods of solving the training objective above. }

1. Model $\Pr(\vg)$ as a mixture of Gaussians with each mixture component as a domain.  A subset of the training domains are used to define the mixture components so that on the remaining the estimated mixture provides a good fit.

2. Another option is to adversarially train $C$ by perturbing only $\vg$.

3. Can we justify cross-gradient as some approximation of the above training objective?




